A fully-coupled framework for solving Cahn-Hilliard Navier-Stokes equations: Second-order, energy-stable numerical methods on adaptive octree based meshes

We present a fully-coupled, implicit-in-time framework for solving a thermodynamically-consistent Cahn-Hilliard Navier-Stokes system that models two-phase flows. In this work, we extend the block iterative method presented in Khanwale et al. [\textit{Simulating two-phase flows with thermodynamically consistent energy stable Cahn-Hilliard Navier-Stokes equations on parallel adaptive octree based meshes}, J. Comput. Phys. (2020)], to a fully-coupled, provably second-order accurate scheme in time, while maintaining energy-stability. The new method requires fewer matrix assemblies in each Newton iteration resulting in faster solution time. The method is based on a fully-implicit Crank-Nicolson scheme in time and a pressure stabilization for an equal order Galerkin formulation. That is, we use a conforming continuous Galerkin (cG) finite element method in space equipped with a residual-based variational multiscale (RBVMS) procedure to stabilize the pressure. We deploy this approach on a massively parallel numerical implementation using parallel octree-based adaptive meshes. We present comprehensive numerical experiments showing detailed comparisons with results from the literature for canonical cases, including the single bubble rise, Rayleigh-Taylor instability, and lid-driven cavity flow problems. We analyze in detail the scaling of our numerical implementation.

==> dendro.tex <==
% !TEX root = methods_paper_withpdfFigures.tex

While the concept of adaptive space partitions is well studied, developing such methods for applications demanding frequent refinements on large distributed systems presents significant challenges. This work builds on existing methods for performing large-scale finite element computations using octree-refined meshes. 
The octree-based framework, \dendro\, is extended to support sub-domains, primarily with the objective of supporting long channels and division of the domain based on arbitrary functions that define the geometry.
We provide a brief description on building the octree mesh in parallel and performing finite element computations. Additional details can be found in~\cite{SundarSampathBiros08}. 
% 
\dendro\ provides the adaptive mesh refinement (AMR) and all parallel data-structures, and for this project, \dendro\ was extended to support domains that are not cuboidal in shape. We give a brief overview of the \dendro\ framework and provide details on the new contributions. The main steps in building and maintaining an adaptively refined mesh in a distributed-memory machine are described below.

\paragraph{Refinement:} The sparse grid is constructed based on the geometry. Proceeding in a top-down fashion, a cell is refined if a surface (defined by a zero level-set of a function, or a cloud of points)  passes through it. 
%
We also provide an additional function that tests for membership and eliminates regions outside the domain. This is necessary as by definition the octree maps to a cuboidal domain. By eliminating regions, we can support arbitrary domains, including domains with holes, such a porous media. 
%
% During the same step, we also determine if the cell is completely inside the pillar, and eliminate it from the mesh in that case.   
Since the refinement happens in an element-local fashion, this step is embarrassingly parallel.
The user passes a function that given coordinates, $x,y,z$ returns the distance from the surface. The eight corners of an octant are tested using this function. If all $8$ points have a positive distance (outside), then we retain this element, but do not refine further. If all $8$ points have a negative distance (inside), then this element is removed from the mesh. If some of the corners of the octant are inside and others outside, then this octant is refined. This is repeated till the desired level of refinement is achieved.  
In distributed memory, all processes start from the root and refine until at least $p$ octants requiring further refinement are produced. Then using a weighted space-filling-curve (SFC) based partitioning, we partition the octants. Note that we do not communicate the octants as every process has a copy of the octants, and all that needs to be done at each process is to retain a subset of the current octants and recurse. Since we use finite element, a 2:1 balancing is enforced following the refinement operation. 

\paragraph{2:1 Balancing:} We enforce a condition in our distributed octrees that no two neighbouring octants differ in size by more than a factor of two. This makes subsequent operations simpler without affecting the adaptive properties. Our balancing algorithm is similar to existing approaches for balancing octrees \cite{bern1999parallel,BursteddeWilcoxGhattas11,SundarSampathAdavaniEtAl07} with the added aspect that it does not generate octants if the ancestor does not exist in the input. This is done to ensure that regions that were previously eliminated are not filled in. The algorithm proposed by \citet{bern1999parallel} is easily extensible to support this case, as we simply need to skip adding balancing octants that violate the criteria.

\paragraph{Partition:} Refinement and the subsequent 2:1 balancing of the octree can result in a non-uniform distribution of elements across the processes, leading to load imbalance. This is particularly challenging when arbitrary geometries are meshed, as this can make the mesh heavily load-imbalanced.  The Morton ordering enables us to equipartition the elements by performing a parallel scan on the number of elements on each process followed by point-to-point communication to redistribute the elements.  As we refine near the two-phase interface, it can affect the performance, as it is likely localized on a small subset of processes, this where Morton ordering comes to rescue and delivers and effective partition. The partitioning scheme is able to handle arbitrary geometries as the partition only tries to equally divide the retained elements across the processes.  The weighted partitioning, is a straightforward extension of our SFC-based partitioning that provides variable weight to the elements based on whether the element lies inside the retained domain of the arbitrary geometry or not. This allows us to more accurately estimate the work on each partition and provide better parallel load-balancing.
 

\paragraph{Meshing:} By meshing we refer to the construction of the (numerical) data structures required for finite element computations from the (topological) octree data. \dendro ~already has efficient implementations for building the required neighbourhood information and for managing overlapping domains between processors (\textit{ghost} or \textit{halo} regions). The key difference with our previous applications is the requirement to handle arbitrary geometries, as all neighbours might not be present in the mesh. This also complicates the process of applying boundary conditions. We added support for defining {\em subdomains} within \dendro. The subdomains are defined using a function that takes a coordinate $(x,y,z)$ as input and returns \texttt{true} or \texttt{false} depending on whether that coordinate is part of the subdomain or not. The subdomain leverages the core mesh data-structure and additionally defines a unique mapping for nodes that are part of the subdomain. It also keeps track of which nodes belong to subdomain boundaries. Therefore, subdomains have a small overhead and store significantly less data than the main mesh data-structure. For our target application, it is important to identify the external (domain) boundary as this dictates which elements will be retained in the domain. Therefore, the subdomain stores two \texttt{bits} to keep track of whether a node is non-boundary, or external. 

\paragraph{Handling hanging nodes:} While the use of quasi-structured grids such as octree-grids makes parallel meshing scalable and efficient, without sacrificing adaptivity, one challenge is to efficiently handle the resulting non-conformity. This results in so called {\em hanging nodes} occurring on faces/edges shared between unequal elements that do not represent independent degrees of freedom. In order to minimize the memory footprint and overall efficiency, the hanging nodes are not stored in \dendro. Instead, since they are constrained by the order of the elements and the non-hanging nodes on the hanging face/edge, we introduce these as temporary variable before elemental matrix assembly or matrix-vector multiplication\footnote{for Matrix-free computations} and eliminate them following the elemental operation. This is fairly straightforward given that our meshes are limited to a 2:1 balance, limiting the number of overall cases to be considered. Additional details on the handling of hanging nodes in \dendro\ can be found in \cite{SundarSampathAdavaniEtAl07}. 

\paragraph{Intergrid transfers}

An essential requirement is to adapt the spatial mesh as the interface moves across the domain. An example of the adaptive mesh refinement following the moving bubble is shown in Figure~\ref{fig:mesh_adaption}. In the distributed memory setting, this also indicates a need to repartition and rebalance the load. Every few time steps, we remesh. This is similar to the initial mesh generation and refinement, except that it is now based on the current position of the interface as well as the original geometry. 
%
This is followed by the 2:1 balance enforcement and meshing. Once the new mesh is generated, we transfer the velocity field from the old mesh to the new mesh using interpolation as needed. Since the intergrid transfer happens only between parent and child (for coarsening and refinement) or remains unchanged, this can be performed on the old mesh using standard polynomial interpolation, followed by a simple repartitioning based on the new mesh (Note that the use of SFCs makes this a linear shift). 
%
% The nodes of the local new mesh are distributed over processes based on the old mesh partitioning to perform interpolation. However again, the intergrid transfer is challenging in unstructured meshes as repartitioning usually offers no guarantee of good overlap between the old and new partitions in most graph-based approaches. The distribution of the nodes of local new mesh would be difficult across complex process boundaries. One way to address it may be to reconstruct the global old mesh in each process, and interpolate for the local new mesh based on the global old mesh, which is memory and time consuming.
